Beyond Discrete Selection: Continuous Embedding Space Optimization for Generative Feature Selection

The goal of Feature Selection - comprising filter, wrapper, and embedded approaches - is to find the optimal feature subset for designated downstream tasks. Nevertheless, current feature selection methods are limited by: 1) the selection criteria of these methods are varied for different domains, making them hard to generalize; 2) the selection performance of these approaches drops significantly when processing high-dimensional feature space coupled with small sample size. In light of these challenges, we pose the question: can selected feature subsets be more robust, accurate, and input dimensionality agnostic? In this paper, we reformulate the feature selection problem as a deep differentiable optimization task and propose a new research perspective: conceptualizing discrete feature subsetting as continuous embedding space optimization. We introduce a novel and principled framework that encompasses a sequential encoder, an accuracy evaluator, a sequential decoder, and a gradient ascent optimizer. This comprehensive framework includes four important steps: preparation of features-accuracy training data, deep feature subset embedding, gradient-optimized search, and feature subset reconstruction. Specifically, we utilize reinforcement feature selection learning to generate diverse and high-quality training data and enhance generalization. By optimizing reconstruction and accuracy losses, we embed feature selection knowledge into a continuous space using an encoder-evaluator-decoder model structure. We employ a gradient ascent search algorithm to find better embeddings in the learned embedding space. Furthermore, we reconstruct feature selection solutions using these embeddings and select the feature subset with the highest performance for downstream tasks as the optimal subset.

==> table/robust_chekc.tex <==
% \begin{table}[!htbp]
% \label{table_robust}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% FS Methods & RF & XGB & SVM & KNN & DT \\
% \midrule
% Raw&0.65 &0.68 &0.63 &0.59 &0.66 \\
% K-Best&0.67 &0.68 &0.61 &0.62 &0.65 \\
% mRMR&0.66 &0.68 &0.61 &0.62 &0.66 \\
% Lasso&0.70 &0.68 &0.65 &0.66 &0.64 \\
% RFE&0.65 &0.67 &0.57$_{\pm0.18}$&0.60 &0.64 \\
% LassoNet&0.58 &0.52 &0.60 &0.55 &0.54 \\
% GFS&0.68 &0.68 &0.64 &0.65 &0.68 \\
% SARLFS&0.63$_{\pm0.09}$&0.64 &0.47$_{\pm0.14}$&0.60 &0.57 \\
% MARLFS&0.69 &0.70 &0.55 &0.64 &0.64$_{\pm0.10}$\\
% RRA&0.70 &0.71 &0.41$_{\pm0.18}$&0.60 &0.67 \\
% MCDM&0.71 &0.69 &0.53 &0.63 &0.66 \\
% \midrule
% \model &\textbf{0.75} &\textbf{0.73} &\textbf{0.71} &\textbf{0.74} &\textbf{0.75} \\
% \bottomrule
% \end{tabular}}
% \end{table}


% \begin{table}[!htbp]
% \label{table_robust}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% FS Methods & RF & XGB & SVM & KNN & DT \\
% \midrule
% Raw&64.88$_{\pm5.99}$&68.01$_{\pm7.88}$&62.73$_{\pm4.46}$&59.02$_{\pm4.67}$&65.94$_{\pm3.17}$\\
% K-Best&66.67$_{\pm5.06}$&67.98$_{\pm4.06}$&61.26$_{\pm6.96}$&62.48$_{\pm5.54}$&65.49$_{\pm6.70}$\\
% mRMR&65.81$_{\pm5.57}$&67.90$_{\pm3.79}$&61.42$_{\pm4.92}$&62.11$_{\pm3.28}$&66.46$_{\pm4.01}$\\
% LASSO&69.65$_{\pm6.21}$&68.16$_{\pm6.65}$&64.53$_{\pm5.63}$&65.86$_{\pm4.26}$&63.57$_{\pm3.76}$\\
% RFE&64.86$_{\pm4.44}$&66.75$_{\pm8.20}$&56.74$_{\pm17.77}$&59.90$_{\pm5.16}$&64.23$_{\pm6.08}$\\
% LASSONet&58.20$_{\pm1.72}$&51.89$_{\pm4.84}$&59.64$_{\pm4.35}$&54.72$_{\pm5.22}$&54.26$_{\pm2.30}$\\
% GFS&67.54$_{\pm3.58}$&67.52$_{\pm4.75}$&63.77$_{\pm3.24}$&64.52$_{\pm2.30}$&68.02$_{\pm5.72}$\\
% SARLFS&63.32$_{\pm8.57}$&64.35$_{\pm6.67}$&47.02$_{\pm13.56}$&60.34$_{\pm6.22}$&57.47$_{\pm7.62}$\\
% MARLFS&69.00$_{\pm3.35}$&69.70$_{\pm2.59}$&54.78$_{\pm13.19}$&63.58$_{\pm4.47}$&63.81$_{\pm9.58}$\\
% RRA&69.69$_{\pm4.33}$&70.63$_{\pm3.70}$&41.15$_{\pm17.99}$&60.37$_{\pm3.66}$&67.01$_{\pm6.93}$\\
% MCDM&70.85$_{\pm3.54}$&68.77$_{\pm3.05}$&53.36$_{\pm13.03}$&62.59$_{\pm5.14}$&65.51$_{\pm4.45}$\\
% \midrule
% \model &\textbf{75.34}$_{\pm6.02}$&\textbf{73.19}$_{\pm6.21}$&\textbf{71.20}$_{\pm7.36}$&\textbf{73.95}$_{\pm6.09}$&\textbf{75.40}$_{\pm5.85}$\\
% \bottomrule
% \end{tabular}}
% \end{table}

\begin{table}[!htbp]
\centering
\caption{Robustness check of \model\ when confronted with distinct downstream ML models in terms of F1-score.}
% \vspace{-0.2cm}
\label{table_robust}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
FS Methods & RF & XGB & SVM & KNN & DT \\
\hline
Raw&64.88&68.01&62.73&59.02&65.94\\\hline
K-Best&66.67&67.98&61.26&62.48&65.49\\\hline
mRMR&65.81&67.90&61.42&62.11&66.46\\\hline
LASSO&69.65&68.16&64.53&65.86&63.57\\\hline
RFE&64.86&66.75&56.74&59.90&64.23\\\hline
LASSONet&58.20&51.89&59.64&54.72&54.26\\\hline
GFS&67.54&67.52&63.77&64.52&68.02\\\hline
SARLFS&63.32&64.35&47.02&60.34&57.47\\\hline
MARLFS&69.00&69.70&54.78&63.58&63.81\\\hline
RRA&69.69&70.63&41.15&60.37&67.01\\\hline
MCDM&70.85&68.77&53.36&62.59&65.51\\\hline
\textbf{\model} &\textbf{75.34}&\textbf{73.19}&\textbf{71.20}&\textbf{73.95}&\textbf{75.40}\\
\hline
\end{tabular}}
% \vspace{-0.4cm}
\end{table}
